Fill-Up: Balancing Long-Tailed Data with Generative Models

Modern text-to-image synthesis models have achieved an exceptional level of photorealism, generating high-quality images from arbitrary text descriptions. In light of the impressive synthesis ability, several studies have exhibited promising results in exploiting generated data for image recognition. However, directly supplementing data-hungry situations in the real-world (e.g. few-shot or long-tailed scenarios) with existing approaches result in marginal performance gains, as they suffer to thoroughly reflect the distribution of the real data. Through extensive experiments, this paper proposes a new image synthesis pipeline for long-tailed situations using Textual Inversion. The study demonstrates that generated images from textual-inverted text tokens effectively aligns with the real domain, significantly enhancing the recognition ability of a standard ResNet50 backbone. We also show that real-world data imbalance scenarios can be successfully mitigated by filling up the imbalanced data with synthetic images. In conjunction with techniques in the area of long-tailed recognition, our method achieves state-of-the-art results on standard long-tailed benchmarks when trained from scratch.

==> Sections/9_ack.tex <==
\begin{ack}

\end{ack}

==> Tables/efficiency_TI.tex <==
\begin{table}[h]
\caption{Comparison with classifier-based GANs.}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lcc}
\cmidrule[1.0pt]{1-3}
\textbf{Method} & Guidance & Top-1\\
\cmidrule[1.0pt]{1-3}
Baseline (ImageNet-LT) & - & 10.2\\
\midrule
Single Template & 7.5 & 10.2 \\
Single Template & 1.0 & 10.2 \\
~+~ ImageNet-LT & 1.0 & 10.2\\
\midrule
Textual Inversion & 1.0 & 10.2\\
~~~+~ ImageNet-LT & 1.0 & 10.2 \\
~+~ 1.3K imgs/cls & 1.0 & 10.2 \\
~+~ ImageNet-LT & 1.0 & 10.2 \\
\midrule
Baseline (Full ImageNet) & - & 10.2\\
\cmidrule[1.0pt]{1-3}
\end{tabular}}
\end{table}
